Online Modifications for Event-based Signal Temporal Logic Specifications

In this paper we present a grammar and control synthesis framework for online modification of Event-based Signal Temporal Logic (STL) specifications, during execution. These modifications allow a user to change the robots' task in response to potential future violations, changes to the environment, or user-defined task design changes. In cases where a modification is not possible, we provide feedback to the user and suggest alternative modifications. We demonstrate our task modification process using a Hello Robot Stretch satisfying an Event-based STL specification.

==> Modifications.tex <==
\section{Online Modifications of Event-based STL Specifications}
\label{sec:onlineControl}


 %We first find the forward B\"{u}chi for all $\gls{buchiset}$. This is the part of the B\"{u}chi that can be reaced at this point in the execution. By calculating this we reduce the computational burden of finding intersections in the future. 
%         \item \textbf{\textit{findMods}} \textbf{(line \ref{line:findMods})}: Given the original specification \gls{psistl} and the modified version of the specification \gls{psinew}, we find all modifications that are made. The modification representing additions to a specification \gls{Gammanew} is a set of tuples $\gls{Gammanew} = \{(\gls{psistl'}_1,\gls{op}_1), (\gls{psistl'}_2,\gls{op}_2),\ldots\}$. Where $\gls{psistl'}_i$ is a specification added to \gls{psistl} and $\gls{op}_i$ is how the specification is added (conjunction or disjunction). Modifications to the timing bounds and predicate of a specification are captured in the set of tuples $\gls{psistlset} = \{(\gls{pinew}^1, \gls{pinew'}^1), (\gls{pinew}^2, \gls{pinew'}^2),\ldots\}$. Where $\gls{pinew}^i$ is the abstracted predicate that is being modified and $\gls{pinew'}^i$ is the newly modified version of $\gls{pinew}^i$.
        
        
%         \item \textbf{\textit{prepSpec}} \textbf{(line \ref{line:prepMod})}: Each added specification \gls{psistil'} is prepared using the same process as the original specification. The output is a set of abstracted propositions $\gls{abstractedpred}^{'}$, B\"{u}chi automata $\gls{buchi}^{'}$, predicate functions $\gls{setpredicatefunc}^{'}$, CBF templates $\gls{cbf}^{'}$, and the initial state $\gls{initialstate}^{'}$ of $\gls{buchi}^{'}$. 
        
%         \item \textbf{(line \ref{line:addPred}-\ref{line:addcbf})} The abstracted propositions $\gls{abstractedpred}^{'}$, predicate functions $\gls{setpredicatefunc}^{'}$, and CBF templates $\gls{cbf}^{'}$ from the new specification are then added to the current sets \gls{abstractedpred}, \gls{setpredicatefunc}, and \gls{cbf}.
%         \item \textbf{\textit{IntersectB}} \textbf{(line \ref{line:buchiIntersect}):} If the new specification is being added via conjunction ($\gls{op} == \wedge$), then a product automaton is found with all $\gls{buchi} \in \gls{buchiset}$. In this case the number of \gls{buchi} in \gls{buchiset} does not change.
%         \item \textbf{(line \ref{line:addbuchi}-\ref{line:addstate})} If the new specification is being added via disjunction ($\gls{op} == \vee$), then $\gls{buchi}^{'}$ and $\gls{initialstate}^{'}$ are added to $\gls{buchi}$ and $\gls{initialstate}$. The decision on which $\gls{buchi} \in \gls{buchiset}$ to follow is made while picking transitions. 
        
        

%         \item \textbf{(line \ref{line:modifyprop})} For each tuple of modified propositions we first determine if the proposition that is modified \gls{pinew} exists in any $\gls{buchi} \in \gls{buchiset}$. If it does exist, then the proposition is modified in the abstracted predicates and execution continues. 
%         \item If the proposition does not exist in any $\gls{buchi} \in \gls{buchiset}$, the desired behavior may not be achieved as the proposition has already been satisfied and will not appear again. 
%         \item \textbf{(line \ref{line:setequal}):} After all modifications are made, the Event-based STL specification is set to be the new specification. This is so that, in subsequent timesteps, new modifications may be added. 
%     \end{itemize}
    
% \end{itemize}



==> Motivating.tex <==
\section{MOTIVATING EXAMPLE}
\hkg{this is really complex}
\subsubsection{Shorthand definitions}
\begin{itemize}
    \item Object position: \\ $\textbf{x}_{obj,t} = [x_{obj,t},y_{obj,t},z_{obj,t}]$
    \item depot position: \\ $\textbf{x}_{dep} = [x_{dep},y_{dep},z_{dep}]$
    \item Robot state:\\  $\textbf{x}_t = [x_t, y_t,\theta_t, d_t, z_t, \beta_t]$
    \\ $d_t$ is the extension of the arm, $z_t$ is the height of the arm, $\beta_t$ is the strength of the grip
\end{itemize}


\subsubsection{Event-based STL}
\begin{itemize}
    \item ``pick up and drop off" task with the stretch
    \item Specification is set up so that modifications can be made on different components
\end{itemize}
\begin{equation}
    \gls{psistl} = G(pickup \rightarrow (\gls{psistl}_1 \wedge \gls{psistl}_2 \wedge \ldots \wedge \gls{psistl}_{11}))
\end{equation}

\begin{itemize}[labelindent=0.5pt,itemindent=0pt,leftmargin=*]
    \item $\gls{psistl}_1 = F_{[0,10]}(\parallel [x_t,y_t] - [x_{obj,t},y_{obj,t}]\parallel < 1)$
    \item $\gls{psistl}_2 = F_{[10,20]}(|\theta_t -tan^{-1}(\frac{y_{obj,t}-y_t}{x_{obj,t}-x_t}) + \frac{\pi}{2}| < 0.1)$
    \item $\gls{psistl}_3 = F_{[10,20]} (|z_t - z_{obj,t}| < 0.05 )$
    \item $\gls{psistl}_4 = F_{[10,20]} (|d_t - \parallel[x_t,y_t] - [x_{obj,t},y_{obj,t}]\parallel| < 0.05 )$
    \item $\gls{psistl}_5 = F_{[20,25]} (\beta_t > 40)$
    \item $\gls{psistl}_6 = F_{[25,35]} (|d_t - 0.1| < 0.1 \wedge |z_t - 1| < 0.1 )$
    \item $\gls{psistl}_7 = F_{[35,45]} (\parallel [x_t,y_t] - [x_{dep},y_{dep}]\parallel < 1)$
    \item $\gls{psistl}_8 = F_{[45,55]}(|\theta_t -tan^{-1}(\frac{y_{dep}-y_t}{x_{dep}-x_t}) + \frac{\pi}{2}| < 0.1)$
    \item $\gls{psistl}_9 = F_{[45,55]} (|z_t - z_{dep}| < 0.05 )$
    \item $\gls{psistl}_{10} = F_{[45,55]} (|d_t - \parallel[x_t,y_t] - [x_{dep},y_{dep}]\parallel| < 0.05 )$
    \item $\gls{psistl}_{11} = F_{[55,60]} (\beta_t < 5)$

\end{itemize}

\begin{itemize}
    \item Specification Overview: 
    \begin{itemize}
        \item If $pickup$ then the stretch must satisfy 11 specifications
        \begin{enumerate}
            \item Navigate to the location of the object to grasp between 0 and 10 seconds.
            \item Within 10-20 seconds the robot must align to the object
            \item Within 10-20 seconds the arm must lower to the height of the object
            \item Within 10-20 seconds the arm must extend to to be within 0.05 units of the object
            \item After the object is within the gripper, within 20-25 seconds the gripper should grasp the object. 
            \item Within 25 and 35 seconds the end effector must retract close to the body of the robot and to a set z position and d position.  
            \item Within 35 and 45 seconds the robot must navigate to the depot
            \item After navigating to the depot. Within 45-55 seconds the robot should align to the depot
            \item Within 45-55 seconds the robot arm must raise to be within 0.05 units of the object height
            \item Within 45-55 seconds the robot arm must extend to be within 0.05 units of the object
            \item Finally, within 55-60 seconds the robot should release the object
        \end{enumerate}
    \end{itemize}
    \item Modifications to be explored
    \begin{itemize}
        \item Timing bounds: If for some reason the object is too far away and the robot can not reach it in time given the control bounds, then a pre-failure warning will be given that the time isn't enough. The user can then edit the timing bound to allow enough time for the robot to make it. 
        \item Predicate: If there is a new $depot$ that the object must be deposited in, then the predicate for the drop off portion off the task can be changed. 
        \item Add through disjunction: Duplicate the entire specification and add it through disjunction. With the change being instead of $depot_1$ it being $depot_2$.
        \item Adding through conjunction: Add the requirement that before the robot deposits the marker it must visit a room out of the way in addition to completing the original task.
    \end{itemize}
\end{itemize}
    
\subsubsection{Stretch Dynamics}
\begin{equation}
    \textbf{x}_t = [x_t, y_t, \theta_t, d_t, z_t, \beta_t]
\end{equation}
\begin{equation}
    \textbf{u}_t = [v_t, \omega_t, v_{d,t}, v_{z,t}, v_{\beta,t}]
\end{equation}
\begin{equation}
g = 
    \begin{bmatrix}
cos(\theta_t) & 0 & 0& 0 & 0\\
sin(\theta_t) & 0 & 0 & 0 & 0\\
0 & 1 & 0 & 0 & 0 \\
0 & 0 & 1 & 0 & 0 \\
0 & 0 & 0 & 1 & 0 \\
0 & 0 & 0 & 0 & 1 
\end{bmatrix}
\end{equation}
% \begin{equation}
%     f(\textbf{x}_t) = I * \textbf{x}_t
% \end{equation}
